Recurrent Neural Networks with Stochastic Layers for Acoustic Novelty Detection

In this paper, we adapt Recurrent Neural Networks with Stochastic Layers, which are the state-of-the-art for generating text, music and speech, to the problem of acoustic novelty detection. By integrating uncertainty into the hidden states, this type of network is able to learn the distribution of complex sequences. Because the learned distribution can be calculated explicitly in terms of probability, we can evaluate how likely an observation is then detect low-probability events as novel. The model is robust, highly unsupervised, end-to-end and requires minimum preprocessing, feature engineering or hyperparameter tuning. An experiment on a benchmark dataset shows that our model outperforms the state-of-the-art acoustic novelty detectors.

==> sections/6_acknowledgement.tex <==
\section{Acknowledgements}
\label{secAcknowledgements}

% {\color{red} I think you dont include acknowledgements in the blind submission, only in the final version. Then include NSERC as well}
The authors would like to thank A3Lab for the dataset. We also acknowledge the UBL Mobility Fund and the Natural Sciences and Engineering Research Council of Canada (NSERC) for the financial support. 


